Search for events with an isolated lepton and missing transverse momentum and a measurement of W production at HERA

A search for events with an isolated high-energy lepton and large missing transverse momentum has been performed with the ZEUS detector at HERA using a total integrated luminosity of 504 $\mathrm{pb}^{-1}$. The results agree well with Standard Model predictions. The cross section for production of single $W$ bosons in electron-proton collisions with unpolarised electrons is measured to be $0.89^{+0.25}_{-0.22}$ (stat.) $\pm{0.10}$ (syst.) pb.

==> auth_list.tex <==
%===================================================================                               
%                                                                                                  
%  MEMBER NAME  AUTH151 (ZEUS)     M  TEX                                                          
%                                                                                                  
%  JH.: transformed to a format, which is suited as input for                                      
%       CONVERT, which automatically creates author-indices                                        
%                                                                                                  
%  Don't remove lines starting with a percent sign %,                                              
%  CONVERT may need them urgently !                                                                
%                                                                                                  
%=====================================================================                             
                                                   %                                               
\begin{center}                                                                                     
{                      \Large  The ZEUS Collaboration              }                               
\end{center}                                                                                       
                                                   %                                               
  S.~Chekanov,                                                                                     
  M.~Derrick,                                                                                      
  S.~Magill,                                                                                       
  B.~Musgrave,                                                                                     
  D.~Nicholass$^{   1}$,                                                                           
  \mbox{J.~Repond},                                                                                
  R.~Yoshida\\                                                                                     
 {\it Argonne National Laboratory, Argonne, Illinois 60439-4815, USA}~$^{n}$                       
\par \filbreak                                                                                     
                                                  %                                                
  M.C.K.~Mattingly \\                                                                              
 {\it Andrews University, Berrien Springs, Michigan 49104-0380, USA}                               
\par \filbreak                                                                                     
  P.~Antonioli,                                                                                    
  G.~Bari,                                                                                         
  L.~Bellagamba,                                                                                   
  D.~Boscherini,                                                                                   
  A.~Bruni,                                                                                        
  G.~Bruni,                                                                                        
  F.~Cindolo,                                                                                      
  M.~Corradi,                                                                                      
\mbox{G.~Iacobucci},                                                                               
  A.~Margotti,                                                                                     
  R.~Nania,                                                                                        
  A.~Polini\\                                                                                      
  {\it INFN Bologna, Bologna, Italy}~$^{e}$                                                        
\par \filbreak                                                                                     
  S.~Antonelli,                                                                                    
  M.~Basile,                                                                                       
  M.~Bindi,                                                                                        
  L.~Cifarelli,                                                                                    
  A.~Contin,                                                                                       
  S.~De~Pasquale$^{   2}$,                                                                         
  G.~Sartorelli,                                                                                   
  A.~Zichichi  \\                                                                                  
{\it University and INFN Bologna, Bologna, Italy}~$^{e}$                                           
\par \filbreak                                                                                     
                                                    %                                              
  D.~Bartsch,                                                                                      
  I.~Brock,                                                                                        
  H.~Hartmann,                                                                                     
  E.~Hilger,                                                                                       
  H.-P.~Jakob,                                                                                     
  M.~J\"ungst,                                                                                     
\mbox{A.E.~Nuncio-Quiroz},                                                                         
  E.~Paul,                                                                                         
  U.~Samson,                                                                                       
  V.~Sch\"onberg,                                                                                  
  R.~Shehzadi,                                                                                     
  M.~Wlasenko\\                                                                                    
  {\it Physikalisches Institut der Universit\"at Bonn,                                             
           Bonn, Germany}~$^{b}$                                                                   
\par \filbreak                                                                                     
                                                  %                                                
  N.H.~Brook,                                                                                      
  G.P.~Heath,                                                                                      
  J.D.~Morris\\                                                                                    
   {\it H.H.~Wills Physics Laboratory, University of Bristol,                                      
           Bristol, United Kingdom}~$^{m}$                                                         
\par \filbreak                                                                                     
  %                                                                                                
  M.~Capua,                                                                                        
  S.~Fazio,                                                                                        
  A.~Mastroberardino,                                                                              
  M.~Schioppa,                                                                                     
  G.~Susinno,                                                                                      
  E.~Tassi  \\                                                                                     
  {\it Calabria University,                                                                        
           Physics Department and INFN, Cosenza, Italy}~$^{e}$                                     
\par \filbreak                                                                                     
                                      %                                                            
  J.Y.~Kim\\                                                                                       
  {\it Chonnam National University, Kwangju, South Korea}                                          
 \par \filbreak                                                                                    
  Z.A.~Ibrahim,                                                                                    
  B.~Kamaluddin,                                                                                   
  W.A.T.~Wan Abdullah\\                                                                            
{\it Jabatan Fizik, Universiti Malaya, 50603 Kuala Lumpur, Malaysia}~$^{r}$                        
 \par \filbreak                                                                                    
  Y.~Ning,                                                                                         
  Z.~Ren,                                                                                          
  F.~Sciulli\\                                                                                     
  {\it Nevis Laboratories, Columbia University, Irvington on Hudson,                               
New York 10027}~$^{o}$                                                                             
\par \filbreak                                                                                     
                                                    %                                              
  J.~Chwastowski,                                                                                  
  A.~Eskreys,                                                                                      
  J.~Figiel,                                                                                       
  A.~Galas,                                                                                        
  M.~Gil,                                                                                          
  K.~Olkiewicz,                                                                                    
  P.~Stopa,                                                                                        
 \mbox{L.~Zawiejski}  \\                                                                           
  {\it The Henryk Niewodniczanski Institute of Nuclear Physics, Polish Academy of Sciences, Cracow,
Poland}~$^{i}$                                                                                     
\par \filbreak                                                                                     
                                                           %                                       
  L.~Adamczyk,                                                                                     
  T.~Bo\l d,                                                                                       
  I.~Grabowska-Bo\l d,                                                                             
  D.~Kisielewska,                                                                                  
  J.~\L ukasik,                                                                                    
  \mbox{M.~Przybycie\'{n}},                                                                        
  L.~Suszycki \\                                                                                   
{\it Faculty of Physics and Applied Computer Science,                                              
           AGH-University of Science and \mbox{Technology}, Cracow, Poland}~$^{p}$                 
\par \filbreak                                                                                     
                                                           %                                       
  A.~Kota\'{n}ski$^{   3}$,                                                                        
  W.~S{\l}omi\'nski$^{   4}$\\                                                                     
  {\it Department of Physics, Jagellonian University, Cracow, Poland}                              
\par \filbreak                                                                                     
                                                           %                                       
  U.~Behrens,                                                                                      
  C.~Blohm,                                                                                        
  A.~Bonato,                                                                                       
  K.~Borras,                                                                                       
  R.~Ciesielski,                                                                                   
  N.~Coppola,                                                                                      
  S.~Fang,                                                                                         
  J.~Fourletova$^{   5}$,                                                                          
  A.~Geiser,                                                                                       
  P.~G\"ottlicher$^{   6}$,                                                                        
  J.~Grebenyuk,                                                                                    
  I.~Gregor,                                                                                       
  T.~Haas,                                                                                         
  W.~Hain,                                                                                         
  A.~H\"uttmann,                                                                                   
  F.~Januschek,                                                                                    
  B.~Kahle,                                                                                        
  I.I.~Katkov,                                                                                     
  U.~Klein$^{   7}$,                                                                               
  U.~K\"otz,                                                                                       
  H.~Kowalski,                                                                                     
  \mbox{E.~Lobodzinska},                                                                           
  B.~L\"ohr,                                                                                       
  R.~Mankel,                                                                                       
  \mbox{I.-A.~Melzer-Pellmann},                                                                    
  \mbox{S.~Miglioranzi},                                                                           
  A.~Montanari,                                                                                    
  T.~Namsoo,                                                                                       
  D.~Notz$^{   8}$,                                                                                
  A.~Parenti,                                                                                      
  L.~Rinaldi$^{   9}$,                                                                             
  P.~Roloff,                                                                                       
  I.~Rubinsky,                                                                                     
  R.~Santamarta$^{  10}$,                                                                          
  \mbox{U.~Schneekloth},                                                                           
  A.~Spiridonov$^{  11}$,                                                                          
  D.~Szuba$^{  12}$,                                                                               
  J.~Szuba$^{  13}$,                                                                               
  T.~Theedt,                                                                                       
  G.~Wolf,                                                                                         
  K.~Wrona,                                                                                        
  \mbox{A.G.~Yag\"ues Molina},                                                                     
  C.~Youngman,                                                                                     
  \mbox{W.~Zeuner}$^{   8}$ \\                                                                     
  {\it Deutsches Elektronen-Synchrotron DESY, Hamburg, Germany}                                    
\par \filbreak                                                                                     
  V.~Drugakov,                                                                                     
  W.~Lohmann,                                                          %                           
  \mbox{S.~Schlenstedt}\\                                                                          
   {\it Deutsches Elektronen-Synchrotron DESY, Zeuthen, Germany}                                   
\par \filbreak                                                                                     
                                                           %                                       
  G.~Barbagli,                                                                                     
  E.~Gallo\\                                                                                       
  {\it INFN Florence, Florence, Italy}~$^{e}$                                                      
\par \filbreak                                                                                     
  P.~G.~Pelfer  \\                                                                                 
  {\it University and INFN Florence, Florence, Italy}~$^{e}$                                       
\par \filbreak                                                                                     
                                                           %                                       
                                                           %                                       
  A.~Bamberger,                                                                                    
  D.~Dobur,                                                                                        
  F.~Karstens,                                                                                     
  N.N.~Vlasov$^{  14}$\\                                                                           
  {\it Fakult\"at f\"ur Physik der Universit\"at Freiburg i.Br.,                                   
           Freiburg i.Br., Germany}~$^{b}$                                                         
\par \filbreak                                                                                     
  P.J.~Bussey$^{  15}$,                                                                            
  A.T.~Doyle,                                                                                      
  W.~Dunne,                                                                                        
  M.~Forrest,                                                                                      
  M.~Rosin,                                                                                        
  D.H.~Saxon,                                                                                      
  I.O.~Skillicorn\\                                                                                
  {\it Department of Physics and Astronomy, University of Glasgow,                                 
           Glasgow, United \mbox{Kingdom}}~$^{m}$                                                  
\par \filbreak                                                                                     
  I.~Gialas$^{  16}$,                                                                              
  K.~Papageorgiu\\                                                                                 
  {\it Department of Engineering in Management and Finance, Univ. of                               
            Aegean, Greece}                                                                        
\par \filbreak                                                                                     
  U.~Holm,                                                                                         
  R.~Klanner,                                                                                      
  E.~Lohrmann,                                                                                     
  P.~Schleper,                                                                                     
  \mbox{T.~Sch\"orner-Sadenius},                                                                   
  J.~Sztuk,                                                                                        
  H.~Stadie,                                                                                       
  M.~Turcato\\                                                                                     
  {\it Hamburg University, Institute of Exp. Physics, Hamburg,                                     
           Germany}~$^{b}$                                                                         
\par \filbreak                                                                                     
  C.~Foudas,                                                                                       
  C.~Fry,                                                                                          
  K.R.~Long,                                                                                       
  A.D.~Tapper\\                                                                                    
   {\it Imperial College London, High Energy Nuclear Physics Group,                                
           London, United \mbox{Kingdom}}~$^{m}$                                                   
\par \filbreak                                                                                     
  T.~Matsumoto,                                                                                    
  K.~Nagano,                                                                                       
  K.~Tokushuku$^{  17}$,                                                                           
  S.~Yamada,                                                                                       
  Y.~Yamazaki$^{  18}$\\                                                                           
  {\it Institute of Particle and Nuclear Studies, KEK,                                             
       Tsukuba, Japan}~$^{f}$                                                                      
\par \filbreak                                                                                     
                                                    %                                              
  A.N.~Barakbaev,                                                                                  
  E.G.~Boos,                                                                                       
  N.S.~Pokrovskiy,                                                                                 
  B.O.~Zhautykov \\                                                                                
  {\it Institute of Physics and Technology of Ministry of Education and                            
  Science of Kazakhstan, Almaty, \mbox{Kazakhstan}}                                                
  \par \filbreak                                                                                   
                                                      %                                            
  V.~Aushev$^{  19}$,                                                                              
  O.~Bachynska,                                                                                    
  M.~Borodin,                                                                                      
  I.~Kadenko,                                                                                      
  A.~Kozulia,                                                                                      
  V.~Libov,                                                                                        
  M.~Lisovyi,                                                                                      
  D.~Lontkovskyi,                                                                                  
  I.~Makarenko,                                                                                    
  Iu.~Sorokin,                                                                                     
  A.~Verbytskyi,                                                                                   
  O.~Volynets\\                                                                                    
  {\it Institute for Nuclear Research, National Academy of Sciences, Kiev                          
  and Kiev National University, Kiev, Ukraine}                                                     
  \par \filbreak                                                                                   
                                                      %                                            
  D.~Son \\                                                                                        
  {\it Kyungpook National University, Center for High Energy Physics, Daegu,                       
  South Korea}~$^{g}$                                                                              
  \par \filbreak                                                                                   
  J.~de~Favereau,                                                                                  
  K.~Piotrzkowski\\                                                                                
  {\it Institut de Physique Nucl\'{e}aire, Universit\'{e} Catholique de                            
  Louvain, Louvain-la-Neuve, \mbox{Belgium}}~$^{q}$                                                
  \par \filbreak                                                                                   
                                                         %                                         
  F.~Barreiro,                                                                                     
  C.~Glasman,                                                                                      
  M.~Jimenez,                                                                                      
  L.~Labarga,                                                                                      
  J.~del~Peso,                                                                                     
  E.~Ron,                                                                                          
  M.~Soares,                                                                                       
  J.~Terr\'on,                                                                                     
  \mbox{M.~Zambrana}\\                                                                             
  {\it Departamento de F\'{\i}sica Te\'orica, Universidad Aut\'onoma                               
  de Madrid, Madrid, Spain}~$^{l}$                                                                 
  \par \filbreak                                                                                   
  F.~Corriveau,                                                                                    
  C.~Liu,                                                                                          
  J.~Schwartz,                                                                                     
  R.~Walsh,                                                                                        
  C.~Zhou\\                                                                                        
  {\it Department of Physics, McGill University,                                                   
           Montr\'eal, Qu\'ebec, Canada H3A 2T8}~$^{a}$                                            
\par \filbreak                                                                                     
                                             %                                                     
  T.~Tsurugai \\                                                                                   
  {\it Meiji Gakuin University, Faculty of General Education,                                      
           Yokohama, Japan}~$^{f}$                                                                 
\par \filbreak                                                                                     
                                                           %                                       
  A.~Antonov,                                                                                      
  B.A.~Dolgoshein,                                                                                 
  D.~Gladkov,                                                                                      
  V.~Sosnovtsev,                                                                                   
  A.~Stifutkin,                                                                                    
  S.~Suchkov \\                                                                                    
  {\it Moscow Engineering Physics Institute, Moscow, Russia}~$^{j}$                                
\par \filbreak                                                                                     
                                                           %                                       
  R.K.~Dementiev,                                                                                  
  P.F.~Ermolov~$^{\dagger}$,                                                                       
  L.K.~Gladilin,                                                                                   
  Yu.A.~Golubkov,                                                                                  
  L.A.~Khein,                                                                                      
 \mbox{I.A.~Korzhavina},                                                                           
  V.A.~Kuzmin,                                                                                     
  B.B.~Levchenko$^{  20}$,                                                                         
  O.Yu.~Lukina,                                                                                    
  A.S.~Proskuryakov,                                                                               
  L.M.~Shcheglova,                                                                                 
  D.S.~Zotkin\\                                                                                    
  {\it Moscow State University, Institute of Nuclear Physics,                                      
           Moscow, Russia}~$^{k}$                                                                  
\par \filbreak                                                                                     
  I.~Abt,                                                                                          
  A.~Caldwell,                                                                                     
  D.~Kollar,                                                                                       
  B.~Reisert,                                                                                      
  W.B.~Schmidke\\                                                                                  
{\it Max-Planck-Institut f\"ur Physik, M\"unchen, Germany}                                         
\par \filbreak                                                                                     
  G.~Grigorescu,                                                                                   
  A.~Keramidas,                                                                                    
  E.~Koffeman,                                                                                     
  P.~Kooijman,                                                                                     
  A.~Pellegrino,                                                                                   
  H.~Tiecke,                                                                                       
  M.~V\'azquez$^{   8}$,                                                                           
  \mbox{L.~Wiggers}\\                                                                              
  {\it NIKHEF and University of Amsterdam, Amsterdam, Netherlands}~$^{h}$                          
\par \filbreak                                                                                     
  N.~Br\"ummer,                                                                                    
  B.~Bylsma,                                                                                       
  L.S.~Durkin,                                                                                     
  A.~Lee,                                                                                          
  T.Y.~Ling\\                                                                                      
  {\it Physics Department, Ohio State University,                                                  
           Columbus, Ohio 43210}~$^{n}$                                                            
\par \filbreak                                                                                     
  P.D.~Allfrey,                                                                                    
  M.A.~Bell,                                                         %                             
  A.M.~Cooper-Sarkar,                                                                              
  R.C.E.~Devenish,                                                                                 
  J.~Ferrando,                                                                                     
  \mbox{B.~Foster},                                                                                
  K.~Korcsak-Gorzo,                                                                                
  K.~Oliver,                                                                                       
  A.~Robertson,                                                                                    
  C.~Uribe-Estrada,                                                                                
  R.~Walczak \\                                                                                    
  {\it Department of Physics, University of Oxford,                                                
           Oxford United Kingdom}~$^{m}$                                                           
\par \filbreak                                                                                     
  A.~Bertolin,                                                         %                           
  F.~Dal~Corso,                                                                                    
  S.~Dusini,                                                                                       
  A.~Longhin,                                                                                      
  L.~Stanco\\                                                                                      
  {\it INFN Padova, Padova, Italy}~$^{e}$                                                          
\par \filbreak                                                                                     
  P.~Bellan,                                                                                       
  R.~Brugnera,                                                                                     
  R.~Carlin,                                                                                       
  A.~Garfagnini,                                                                                   
  S.~Limentani\\                                                                                   
  {\it Dipartimento di Fisica dell' Universit\`a and INFN,                                         
           Padova, Italy}~$^{e}$                                                                   
\par \filbreak                                                                                     
                                                           %                                       
  B.Y.~Oh,                                                                                         
  A.~Raval,                                                                                        
  J.~Ukleja$^{  21}$,                                                                              
  J.J.~Whitmore$^{  22}$\\                                                                         
  {\it Department of Physics, Pennsylvania State University,                                       
           University Park, Pennsylvania 16802}~$^{o}$                                             
\par \filbreak                                                                                     
                                                           %                                       
  Y.~Iga \\                                                                                        
{\it Polytechnic University, Sagamihara, Japan}~$^{f}$                                             
\par \filbreak                                                                                     
                                                           %                                       
  G.~D'Agostini,                                                                                   
  G.~Marini,                                                                                       
  A.~Nigro \\                                                                                      
  {\it Dipartimento di Fisica, Universit\`a 'La Sapienza' and INFN,                                
           Rome, Italy}~$^{e}~$                                                                    
\par \filbreak                                                                                     
                                                           %                                       
  J.E.~Cole$^{  23}$,                                                                              
  J.C.~Hart\\                                                                                      
  {\it Rutherford Appleton Laboratory, Chilton, Didcot, Oxon,                                      
           United Kingdom}~$^{m}$                                                                  
\par \filbreak                                                                                     
                          %                                                           %            
  H.~Abramowicz$^{  24}$,                                                                          
  R.~Ingbir,                                                                                       
  S.~Kananov,                                                                                      
  A.~Levy,                                                                                         
  A.~Stern\\                                                                                       
  {\it Raymond and Beverly Sackler Faculty of Exact Sciences,                                      
School of Physics, Tel Aviv University, Tel Aviv, Israel}~$^{d}$                                   
\par \filbreak                                                                                     
                                                           %                                       
  M.~Kuze,                                                                                         
  J.~Maeda \\                                                                                      
  {\it Department of Physics, Tokyo Institute of Technology,                                       
           Tokyo, Japan}~$^{f}$                                                                    
\par \filbreak                                                                                     
  R.~Hori,                                                                                         
  S.~Kagawa$^{  25}$,                                                                              
  N.~Okazaki,                                                                                      
  S.~Shimizu,                                                                                      
  T.~Tawara\\                                                                                      
  {\it Department of Physics, University of Tokyo,                                                 
           Tokyo, Japan}~$^{f}$                                                                    
\par \filbreak                                                                                     
                                                           %                                       
  R.~Hamatsu,                                                                                      
  H.~Kaji$^{  26}$,                                                                                
  S.~Kitamura$^{  27}$,                                                                            
  O.~Ota$^{  28}$,                                                                                 
  Y.D.~Ri\\                                                                                        
  {\it Tokyo Metropolitan University, Department of Physics,                                       
           Tokyo, Japan}~$^{f}$                                                                    
\par \filbreak                                                                                     
                                                           %                                       
  M.~Costa,                                                                                        
  M.I.~Ferrero,                                                                                    
  V.~Monaco,                                                                                       
  R.~Sacchi,                                                                                       
  A.~Solano\\                                                                                      
  {\it Universit\`a di Torino and INFN, Torino, Italy}~$^{e}$                                      
\par \filbreak                                                                                     
  M.~Arneodo,                                                                                      
  M.~Ruspa\\                                                                                       
 {\it Universit\`a del Piemonte Orientale, Novara, and INFN, Torino,                               
Italy}~$^{e}$                                                                                      
                                                           %                                       
\par \filbreak                                                                                     
                                    %                                                              
  S.~Fourletov$^{   5}$,                                                                           
  J.F.~Martin,                                                                                     
  T.P.~Stewart\\                                                                                   
   {\it Department of Physics, University of Toronto, Toronto, Ontario,                            
Canada M5S 1A7}~$^{a}$                                                                             
\par \filbreak                                                                                     
  S.K.~Boutle$^{  16}$,                                                                            
  J.M.~Butterworth,                                                                                
  C.~Gwenlan$^{  29}$,                                                                             
  T.W.~Jones,                                                                                      
  J.H.~Loizides,                                                                                   
  M.~Wing$^{  30}$  \\                                                                             
  {\it Physics and Astronomy Department, University College London,                                
           London, United \mbox{Kingdom}}~$^{m}$                                                   
\par \filbreak                                                                                     
                                                           %                                       
  B.~Brzozowska,                                                                                   
  J.~Ciborowski$^{  31}$,                                                                          
  G.~Grzelak,                                                                                      
  P.~Kulinski,                                                                                     
  P.~{\L}u\.zniak$^{  32}$,                                                                        
  J.~Malka$^{  32}$,                                                                               
  R.J.~Nowak,                                                                                      
  J.M.~Pawlak,                                                                                     
  \mbox{T.~Tymieniecka,}                                                                           
  A.~Ukleja,                                                                                       
  A.F.~\.Zarnecki \\                                                                               
   {\it Warsaw University, Institute of Experimental Physics,                                      
           Warsaw, Poland}                                                                         
\par \filbreak                                                                                     
                                                           %                                       
  M.~Adamus,                                                                                       
  P.~Plucinski$^{  33}$\\                                                                          
  {\it Institute for Nuclear Studies, Warsaw, Poland}                                              
\par \filbreak                                                                                     
                                                           %                                       
  Y.~Eisenberg,                                                                                    
  D.~Hochman,                                                                                      
  U.~Karshon\\                                                                                     
    {\it Department of Particle Physics, Weizmann Institute, Rehovot,                              
           Israel}~$^{c}$                                                                          
\par \filbreak                                                                                     
  E.~Brownson,                                                                                     
  T.~Danielson,                                                                                    
  A.~Everett,                                                                                      
  D.~K\c{c}ira,                                                                                    
  D.D.~Reeder,                                                                                     
  P.~Ryan,                                                                                         
  A.A.~Savin,                                                                                      
  W.H.~Smith,                                                                                      
  H.~Wolfe\\                                                                                       
  {\it Department of Physics, University of Wisconsin, Madison,                                    
Wisconsin 53706}, USA~$^{n}$                                                                       
\par \filbreak                                                                                     
                                                           %                                       
  S.~Bhadra,                                                                                       
  C.D.~Catterall,                                                                                  
  Y.~Cui,                                                                                          
  G.~Hartner,                                                                                      
  S.~Menary,                                                                                       
  U.~Noor,                                                                                         
  J.~Standage,                                                                                     
  J.~Whyte\\                                                                                       
  {\it Department of Physics, York University, Ontario, Canada M3J                                 
1P3}~$^{a}$                                                                                        
                                                           %                                       
\newpage                                                                                           
\enlargethispage{5cm}                                                                              
                                                           %                                       
$^{\    1}$ also affiliated with University College London,                                        
United Kingdom\\                                                                                   
$^{\    2}$ now at University of Salerno, Italy \\                                                 
$^{\    3}$ supported by the research grant no. 1 P03B 04529 (2005-2008) \\                        
$^{\    4}$ This work was supported in part by the Marie Curie Actions Transfer of Knowledge       
project COCOS (contract MTKD-CT-2004-517186)\\                                                     
$^{\    5}$ now at University of Bonn, Germany \\                                                  
$^{\    6}$ now at DESY group FEB, Hamburg, Germany \\                                             
$^{\    7}$ now at University of Liverpool, UK \\                                                  
$^{\    8}$ now at CERN, Geneva, Switzerland \\                                                    
$^{\    9}$ now at Bologna University, Bologna, Italy \\                                           
$^{  10}$ now at BayesForecast, Madrid, Spain \\                                                   
$^{  11}$ also at Institut of Theoretical and Experimental                                         
Physics, Moscow, Russia\\                                                                          
$^{  12}$ also at INP, Cracow, Poland \\                                                           
$^{  13}$ also at FPACS, AGH-UST, Cracow, Poland \\                                                
$^{  14}$ partly supported by Moscow State University, Russia \\                                   
$^{  15}$ Royal Society of Edinburgh, Scottish Executive Support Research Fellow \\                
$^{  16}$ also affiliated with DESY, Germany \\                                                    
$^{  17}$ also at University of Tokyo, Japan \\                                                    
$^{  18}$ now at Kobe University, Japan \\                                                         
$^{  19}$ supported by DESY, Germany \\                                                            
$^{  20}$ partly supported by Russian Foundation for Basic                                         
Research grant no. 05-02-39028-NSFC-a\\                                                            
$^{  21}$ partially supported by Warsaw University, Poland \\                                      
$^{  22}$ This material was based on work supported by the                                         
National Science Foundation, while working at the Foundation.\\                                    
$^{  23}$ now at University of Kansas, Lawrence, USA \\                                            
$^{  24}$ also at Max Planck Institute, Munich, Germany, Alexander von Humboldt                    
Research Award\\                                                                                   
$^{  25}$ now at KEK, Tsukuba, Japan \\                                                            
$^{  26}$ now at Nagoya University, Japan \\                                                       
$^{  27}$ member of Department of Radiological Science,                                            
Tokyo Metropolitan University, Japan\\                                                             
$^{  28}$ now at SunMelx Co. Ltd., Tokyo, Japan \\                                                 
$^{  29}$ PPARC Advanced fellow \\                                                                 
$^{  30}$ also at Hamburg University, Inst. of Exp. Physics,                                       
Alexander von Humboldt Research Award and partially supported by DESY, Hamburg, Germany\\          
$^{  31}$ also at \L\'{o}d\'{z} University, Poland \\                                              
$^{  32}$ member of \L\'{o}d\'{z} University, Poland \\                                            
$^{  33}$ now at Lund Universtiy, Lund, Sweden \\                                                  
                                                           %                                       
$^{\dagger}$ deceased \\                                                                           
%                                                                                                  
% \par         % if index listing & table fit to 1 page, put gap here                              
\newpage   % alternatively: go to newpage, if page is too small                                    
                                                           %                                       
% \institute_references_start    % do not touch or move this line !                                
                                                           %                                       
\begin{tabular}[h]{rp{14cm}}                                                                       
                                                           %                                       
$^{a}$ &  supported by the Natural Sciences and Engineering Research Council of Canada (NSERC) \\  
$^{b}$ &  supported by the German Federal Ministry for Education and Research (BMBF), under        
          contract numbers 05 HZ6PDA, 05 HZ6GUA, 05 HZ6VFA and 05 HZ4KHA\\                         
$^{c}$ &  supported in part by the MINERVA Gesellschaft f\"ur Forschung GmbH, the Israel Science   
          Foundation (grant no. 293/02-11.2) and the U.S.-Israel Binational Science Foundation \\  
$^{d}$ &  supported by the Israel Science Foundation\\                                             
$^{e}$ &  supported by the Italian National Institute for Nuclear Physics (INFN) \\                
$^{f}$ &  supported by the Japanese Ministry of Education, Culture, Sports, Science and Technology 
          (MEXT) and its grants for Scientific Research\\                                          
$^{g}$ &  supported by the Korean Ministry of Education and Korea Science and Engineering          
          Foundation\\                                                                             
$^{h}$ &  supported by the Netherlands Foundation for Research on Matter (FOM)\\                   
$^{i}$ &  supported by the Polish State Committee for Scientific Research, project no.             
          DESY/256/2006 - 154/DES/2006/03\\                                                        
$^{j}$ &  partially supported by the German Federal Ministry for Education and Research (BMBF)\\   
$^{k}$ &  supported by RF Presidential grant N 8122.2006.2 for the leading                         
          scientific schools and by the Russian Ministry of Education and Science through its      
          grant for Scientific Research on High Energy Physics\\                                   
$^{l}$ &  supported by the Spanish Ministry of Education and Science through funds provided by     
          CICYT\\                                                                                  
$^{m}$ &  supported by the Science and Technology Facilities Council, UK\\                         
$^{n}$ &  supported by the US Department of Energy\\                                               
$^{o}$ &  supported by the US National Science Foundation. Any opinion,                            
findings and conclusions or recommendations expressed in this material                             
are those of the authors and do not necessarily reflect the views of the                           
National Science Foundation.\\                                                                     
$^{p}$ &  supported by the Polish Ministry of Science and Higher Education                         
as a scientific project (2006-2008)\\                                                              
$^{q}$ &  supported by FNRS and its associated funds (IISN and FRIA) and by an Inter-University    
          Attraction Poles Programme subsidised by the Belgian Federal Science Policy Office\\     
$^{r}$ &  supported by the Malaysian Ministry of Science, Technology and                           
Innovation/Akademi Sains Malaysia grant SAGA 66-02-03-0048\\                                       
%                                                                                                  
\end{tabular}                                                                                      
                                                           %                                       
% \institute_references_end     % do not touch or move this line !                                 
                                                           %                                       


